MOTSynth: How Can Synthetic Data Help Pedestrian Detection and Tracking?

Deep learning-based methods for video pedestrian detection and tracking require large volumes of training data to achieve good performance. However, data acquisition in crowded public environments raises data privacy concerns -- we are not allowed to simply record and store data without the explicit consent of all participants. Furthermore, the annotation of such data for computer vision applications usually requires a substantial amount of manual effort, especially in the video domain. Labeling instances of pedestrians in highly crowded scenarios can be challenging even for human annotators and may introduce errors in the training data. In this paper, we study how we can advance different aspects of multi-person tracking using solely synthetic data. To this end, we generate MOTSynth, a large, highly diverse synthetic dataset for object detection and tracking using a rendering game engine. Our experiments show that MOTSynth can be used as a replacement for real data on tasks such as pedestrian detection, re-identification, segmentation, and tracking.

==> tables/dataset_comparison_small.tex <==
\begin{table}[t]
\begin{center}
\small
\setlength\tabcolsep{2pt}
\begin{tabular}{lrrccccc}
\toprule
\noalign{\smallskip}
Dataset                                     & \#Frames  & \#Inst.   & 3D    & Pose & Segm.   & Depth \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
PoseTrack~\cite{andriluka2018posetrack} 	& 46k	& 276k 	    &       & \ckm      &               &                     	    \\
MOTS~\cite{Voigtlaender19CVPR}              & 2k	& 26k        &       &           & \ckm          &                	            \\
MOT-17~\cite{Milan16arxiv} 		        & 11k 	& 292k 	    &       & 			&               &                      	    \\
MOT-20~\cite{dendorfer2020mot20} 			& 13k	& 1,652k	&       & 			&               &                      	    \\

\noalign{\smallskip}
\midrule
\noalign{\smallskip}
VIPER~\cite{kim20cvpr}                      & 254k  & 2,750k     & \ckm  &           & \ckm          &               	        \\
GTA~\cite{krahenbuhl2018free}               & 250k   & 3,875k    &       &           & \ckm          & \ckm          	        \\

JTA~\cite{fabbri2018learning}               & 460k	& 15,341k    & \ckm	& \ckm      &               &                      	    \\
\midrule
\midrule
\motsynth 					                & 1,382k	& 40,780k 	& \ckm	& \ckm      & \ckm          &\ckm           	        \\
\bottomrule
\end{tabular}
\vspace{-7pt}
\caption[Publicly available datasets]{Overview of the publicly available datasets for pedestrian detection and tracking. For each dataset, we report the numbers of annotated frames and instances, as well as the availability of different labels.}
\label{table:datasets_small}
\end{center}
\end{table}

==> tables/detection/detection_bench.tex <==
\begin{table}
\center
\tabcolsep=0.11cm
\resizebox{\columnwidth}{!}{
\begin{tabular}{c| l| c c c |c c c| c c c c c}
\toprule
& Dataset & AP $\uparrow$ & MODA $\uparrow$ & FAF $\downarrow$ & TP $\uparrow$ & FP $\downarrow$ & FN $\downarrow$ & Rec. $\uparrow$ & Pr. $\uparrow$  \\ [0.5ex] 
 \midrule

\parbox[t]{3mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{MOT17}}} 
& ZIZOM~\cite{lin2018graininess} & \textbf{0.81} & 72.0 & 2.2 & 95414 & 12990 & 19139 & 83.3 & 88.0\\
& SDP~\cite{Yang16CVPR} & \textbf{0.81} & \textbf{76.9} & \textbf{1.3} & 95699 & \textbf{7599} & 18865 & 83.5 & \textbf{92.6}\\
& DPM~\cite{Felzenszwalb08CVPR} & 0.61 & 31.2 & 7.1 & 78007 & 42308 & 36557 & 68.1 & 64.8\\

& FRCNN~\cite{Ren15NIPS} & 0.72 & 68.5 & 1.7 & 88601 & 10081 & 25963 & 77.3 & 89.8\\
\cline{2-10}
& FRCNN \motsynth & 0.80 & 66.7 & 3.7 & 98164 & 21748 & 16400  & 81.9 & 83.7 \\
& FRCNN \motsynth + FT & 0.80 & 71.0 & 3.5 & \textbf{102341} & 20989 & \textbf{12223} & \textbf{89.3} & 83.0 \\
\midrule
\parbox[t]{3mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{MOT20}}} 
& GNN\_SDT~\cite{wang2020joint} & \textbf{0.81} & \textbf{79.3} & 7.1 & \textbf{304236} & 31677 & \textbf{39288} & \textbf{88.6} & 90.6\\
& VIPeD20~\cite{ciampi2020virtual} & 0.80 & 46.0 & 31.1 & 297101 & 139111 & 46277 & 86.5 & 68.1\\
\cline{2-10}
& FRCNN \motsynth & 0.62 & 52.0 & 6.3 & 206902 & 28202 & 136622 & 60.2 & 88.0 \\
& FRCNN \motsynth + FT & 0.72 & 63.3 & \textbf{5.2} & 241056 & \textbf{23465} & 102468 & 70.2 & \textbf{91.1} \\


\bottomrule
\end{tabular}}
\vspace{-7pt}
\caption{We train Faster R-CNN on \motsynth with and without fine-tuning and evaluate on MOTChallenge MOT17 and MOT20 pedestrian detection test sets.}
\label{tab:detection-bench}
\end{table}



==> tables/detection/detection_comparison.tex <==
\begin{table}
\center
\tabcolsep=0.11cm
\resizebox{\columnwidth}{!}{
\begin{tabular}{c| l| c c c |c c c| c c c c c}
\toprule
& Dataset & AP $\uparrow$ & MODA $\uparrow$ & FAF $\downarrow$ & TP $\uparrow$ & FP $\downarrow$ & FN $\downarrow$ & Rec. $\uparrow$ & Pr. $\uparrow$  \\ [0.5ex] 
 \midrule
\parbox[t]{3mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\footnotesize YOLOv3}}} 
& VIPER & 26.65 & 22.02 & \textbf{0.16} & 15447 & \textbf{838} & 50910 & 23.28 & \textbf{94.85}\\
& JTA & 53.18 & 48.77 & 0.79 & 36578 & 4200 & 29815 & 55.09 & 89.70\\
& \motsynth--256 & 62.99 & 62.31 & 0.58 & 44458 & 3090 & 21935 & 66.96 & 93.50 \\
& \textbf{\motsynth-full} & 71.90 & 64.51 & 1.07 & \textbf{48500} & 5673 & \textbf{17893} & \textbf{73.05} & 89.53 \\
\midrule
\parbox[t]{3mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\footnotesize CenterNet}}} 
& VIPER & 44.58 & 36.92 & \textbf{1.24} & 31122 & \textbf{6611} & 35271 & 46.88 & \textbf{82.48}\\
& JTA & 60.15 & 45.38 & 2.32 & 42435 & 12308 & 23958 & 63.91 & 77.52\\
& \motsynth--256 & 61.82 & 50.11 & 2.03 & 44067 & 10795 & 22326 & 66.37 & 80.32 \\
& \textbf{\motsynth-full} & \textbf{70.49} & \textbf{55.25} & 2.11 & \textbf{47883} & 11204 & \textbf{18510} & \textbf{72.12} & 81.04 \\
\midrule
\parbox[t]{3mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\footnotesize Faster R-CNN}}} 
& VIPER & 60.93 & 42.87 &\textbf{ 2.87} & 43707 & \textbf{15241} & \textbf{10593} & 65.82 & 74.14\\
& JTA & 69.69 & 38.38 & 5.12 & 52726 & 27242 & 13667 & 65.93 & \textbf{79.41}\\
& \motsynth--256 & 78.61 & \textbf{58.65} & 3.10 & \textbf{55441} & 16504 & 10952 & \textbf{83.50} & 77.06 \\
& \textbf{\motsynth-full} & \textbf{78.98} & 54.96 & 3.51 & 55121 & 18634 & 11272 & 83.02 & 74.74 \\
\bottomrule
\end{tabular}}
\vspace{-7pt}
\caption{Comparison on MOT17 against synthetic datasets.}
\label{tab:detection-dataset-comparison}
\end{table}



==> tables/detection/detectors_mot17.tex <==
\begin{table*}
\center
\tabcolsep=0.11cm
\resizebox{\textwidth}{!}{
\begin{tabular}{c | c | l| c c c| c c c| c c c c c|}
\toprule
& & Dataset & AP $\uparrow$ & MODA $\uparrow$ & FAF $\downarrow$ & TP $\uparrow$ & FP $\downarrow$ & FN $\downarrow$ & Rec. $\uparrow$ & Pr. $\uparrow$  \\ [0.5ex] 
\midrule
\parbox[t]{3mm}{\multirow{20}{*}{\rotatebox[origin=c]{90}{\textbf{MOT17}}}} &
\parbox[t]{3mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{YOLOv3}}} 
 
& COCO & 69.76 & 62.02 & 1.25 & 47824 & 6650 & 18569 & 72.03 & 87.79\\
\cline{3-11}
& & \motsynth--1 & 62.66 & 52.36 & 1.43 & 42378 & 7613 & 24015 & 63.83 & 84.77 \\
& & \motsynth--2 & 63.08 & 56.67 & 1.22 & 44116 & 6489 & 22277 & 66.45 & 87.18 \\
& & \motsynth--3 & 63.13 & 60.60 & 1.13 & 46264 & 6029 & 20129 & 69.68 & 88.47 \\
& & \motsynth--4 & \textbf{71.90} & \textbf{64.51} & \textbf{1.07} & \textbf{48500} & \textbf{5673} & \textbf{17893} & \textbf{73.05} & \textbf{89.53} \\
\cline{2-11}
& \parbox[t]{3mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{CenterNet}}} 
& COCO & 67.01 & 44.38 & 3.37 & 47398 & 17935 & 18995 & 71.39 & 72.55\\
\cline{3-11}
& & \motsynth--1 & 61.82 & 49.34 & 2.04 & 43626 & 10866 & 22767 & 65.71 & 80.06 \\
& & \motsynth--2 & 62.32 & 54.90 & \textbf{1.66} & 45269 & \textbf{8820}  & 21124 & 68.18 & \textbf{83.69} \\
& & \motsynth--3 & 62.45 & 55.82 & 1.72 & 46177 & 9117  & 20216 & 69.55 & 83.51 \\
& & \motsynth--4 & \textbf{70.68} & \textbf{57.39} & 1.81 & \textbf{47748} & 9646  & \textbf{18645} & \textbf{71.92} & 83.19 \\
\cline{2-11}
& \parbox[t]{3mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{Faster R-CNN}}} 
& COCO & 76.68 & 53.86 & \textbf{3.45} & 54127 & \textbf{18364} & 12266 & 81.52 & 74.67\\
\cline{3-11}
& & \motsynth--1 & 76.80 & 39.02 & 5.19 & 53507 & 27603 & 12886 & 80.59 & 65.97 \\
& & \motsynth--2 & 77.47 & 50.62 & 3.82 & 53893 & 20287 & 12500 & 81.17 & 72.65 \\
& & \motsynth--3 & 78.31 & 49.75 & 4.22 & \textbf{55474} & 22441 & \textbf{10919} & \textbf{83.55} & 71.20 \\
& & \motsynth--4 & \textbf{78.98} & \textbf{54.96} & 3.51 & 55121 & 18634 & 11272 & 83.02 & \textbf{74.74} \\
\cline{2-11}
& \parbox[t]{3mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{Mask R-CNN}}} 
& COCO & 76.96 & 55.55 & 3.31 & 54502 & 17620 & 11891 & 82.09 & 75.57\\
\cline{3-11}
& & \motsynth--1 & 77.58 & 38.43 & 5.51 & 54817 & 29299 & 11576 & 82.56 & 65.17 \\
& & \motsynth--2 & 77.88 & 50.01 & 4.09 & 54930 & 21724 & 11463 & 82.73 & 71.66 \\
& & \motsynth--3 & 78.08 & 49.85 & 4.14 & \textbf{55096} & 21998 & \textbf{11297} & \textbf{82.98} & 71.47 \\
& & \motsynth--4 & \textbf{78.83} & \textbf{56.61} & \textbf{3.17} & 54461 & \textbf{16874} & 11932 & 82.03 & \textbf{76.35} \\
\bottomrule
\end{tabular}
\begin{tabular}{|c | c| l| c c c |c c c| c c }
\toprule
& & Dataset & AP $\uparrow$ & MODA $\uparrow$ & FAF $\downarrow$ & TP $\uparrow$ & FP $\downarrow$ & FN $\downarrow$ & Rec. $\uparrow$ & Pr. $\uparrow$  \\ [0.5ex] 
\midrule
\parbox[t]{3mm}{\multirow{20}{*}{\rotatebox[origin=c]{90}{\textbf{MOT20}}}} &
\parbox[t]{3mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{YOLOv3}}} 
& COCO & 42.42 & 35.10 & 6.88 & 381635 & 61446 & 530602 & 41.84 & 86.13\\
\cline{3-11}
& & \motsynth--1 & 35.83 & 31.15 & \textbf{2.57} & 307127 & \textbf{22956} & 605110 & 33.67 & 93.05 \\
& & \motsynth--2 & 44.49 & 38.01 & 3.25 & 375739 & 29033 & 536498 & 41.19 & 92.83 \\
& & \motsynth--3 & 44.68 & 42.89 & 3.56 & 423029 & 31797 & 489208 & 46.37 & 93.01 \\
& & \motsynth--4 & \textbf{53.69} & \textbf{48.87} & 2.87 & \textbf{471395} & 25621 & \textbf{440842} & \textbf{51.67} & \textbf{94.85} \\
\cline{2-11}
& \parbox[t]{3mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{CenterNet}}} 
& COCO & 39.39 & 28.75 & 12.38 & 372835 & 110537 & 539402 & 40.87 & 77.13\\
\cline{3-11}
& & \motsynth--1 & 43.35 & 30.84 & 16.21 & 426095 & 144781 & 486142 & 46.71 & 74.64 \\
& & \motsynth--2 & 43.76 & 40.23 & 7.27 & 431932 & 64971 & 480305 & 47.35 & \textbf{86.92} \\
& & \motsynth--3 & 34.08 & 24.29 & \textbf{6.72} & 281596 & \textbf{60002} & 630641 & 30.87 & 82.43 \\
& & \motsynth--4 & \textbf{51.70} & \textbf{42.18} & 9.72 & \textbf{471592} & 86787 & \textbf{440645} & \textbf{51.70} & 84.46 \\
\cline{2-11}
& \parbox[t]{3mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{Faster R-CNN}}} 
& COCO & 43.67 & 40.55 & 5.90 & 422649 & 52698 & 489588 & 46.33 & 88.91\\
\cline{3-11}
& & \motsynth--1 & 52.96 & 46.72 & 8.80 & 504790 & 78575 & 407447 & 55.34 & 86.53 \\
& & \motsynth--2 & 52.56 & 46.96 & 7.91 & 498967 & 70609 & 413270 & 54.70 & 87.60 \\
& & \motsynth--3 & 53.37 & 51.38 & 6.36 & 525547 & 56799 & 386690 & 57.61 & 90.25 \\
& & \motsynth--4 & \textbf{53.90} & \textbf{56.03} & \textbf{3.724} & \textbf{544416} & \textbf{33259} & \textbf{367821} & \textbf{59.67} & \textbf{94.25} \\
\cline{2-11}
& \parbox[t]{3mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{Mask R-CNN}}} 
& COCO & 43.73 & 41.99 & 6.39 & 440081 & 57046 & 472156 & 48.24 & 88.52\\
\cline{3-11}
& & \motsynth--1 & 52.75 & 44.98 & 10.28 & 502154 & 91819 & 410483 & 55.05 & 84.54 \\
& & \motsynth--2 & 53.13 & 50.17 & 6.63 & 516896 & 59225 & 395341 & 56.66 & 89.72 \\
& & \motsynth--3 & 53.51 & 52.27 & 5.76 & 528230 & 51408 & 384007 & 57.90 & 91.13 \\
& & \motsynth--4 & \textbf{54.03} & \textbf{55.69} & \textbf{4.11} & \textbf{544703} & \textbf{36715} & \textbf{367534} & \textbf{59.71} & \textbf{93.69} \\
\bottomrule
\end{tabular}
}
\vspace{-7pt}
\caption{To perform synth-to-real control experiment, we train several object detector models on COCO dataset and on four \motsynth subsets. We evaluate all models on MOTChallenge MOT17 (\textit{left}) and MOT20 (\textit{right}) detection datasets. We observe a clear trend with all object detectors: by purely training on synthetic data, we obtain better performance compared to training on a real-world dataset.}
\label{tab:detection-mot17}
\end{table*}



==> tables/reid.tex <==
\begin{table}[t]
\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c|l|c|c|c}
\toprule
& Dataset  & Split & mAP & Rank1\\
\midrule
\parbox[t]{3mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Real}}} 
& Market1501~\cite{zheng2015scalable} & -- & 64.6  & 91.9\\
& Market1501~\cite{zheng2015scalable} + CUHK03~\cite{li2014deepreid} & -- & 69.1 & 91.9\\
\midrule
\parbox[t]{3mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Synthetic}}} 
& \multirow{4}{*}{\motsynth}  & 1 & 71.3 & 91.4\\
&  & 2 & 73.1 & 91.8 \\
&  & 3 &  74.2 & 92.6 \\
&  & 4 &  \textbf{75.2} & \textbf{92.8} \\

\bottomrule
\end{tabular}
}
\vspace{-7pt}
\caption{Person ReID experiments on MOT17.} %
\label{tab:reid}
\end{table}


==> tables/tracking/mot-bench.tex <==
\begin{table}
\center
\tabcolsep=0.11cm
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|l| c c c | c c c}
\toprule
& Method & MOTA $\uparrow$ & MOTP $\uparrow$ & IDF1 $\uparrow$ & FP $\downarrow$ & FN $\downarrow$ & IDS $\downarrow$  \\ [0.5ex] 
\midrule
\parbox[t]{3mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{MOT17}}} 
& Tracktor-\motsynth & 56.9 & 78.0 & 56.9 & 20852 & 220273 & 2012 \\
& Tracktor-\motsynth + FT & 59.1 & 79.3 & 58.8 & 22231 & 206062 & 2323 \\
& Tracktor~\cite{Bergmann19ICCV} & 53.5 & 78.0 & 52.3 & 12201 & 248047 & 2072  \\
& Tracktorv2~\cite{Bergmann19ICCV} & 56.3 & 78.8 & 55.1 & \textbf{8866} & 235449 & 1987 \\
\cline{2-8}
& CenterTrack-\motsynth & 59.7 & 77.4 & 52.0 & 39707 & 181471 & 6035 \\
& CenterTrack-\motsynth + FT & \textbf{65.1} & \textbf{79.9} & 57.9 & 11521 & \textbf{180901} & 4377 \\
& CenterTrack~\cite{zhou20ECCV} & 61.5 & 78.9 & 59.6 & 14076 & 200672 & 2583 \\
\cline{2-8}


& Lif\_T~\cite{hornakova20ICML} & 60.5 & 78.3 & 65.6 & 14966 & 206619 & 1189  \\
& LPC~\cite{dai2021learning} & 59.0 & 78.0 &\textbf{ 66.8} & 23102 & 206948 & \textbf{1122}  \\
& MPNTrack~\cite{braso2020learning} & 58.8 & 78.6 & 61.7 & 17413 & 213594 & 1185  \\

\midrule
\midrule
\parbox[t]{3mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{MOT20}}} 
& Tracktor-\motsynth & 43.7 & 75.1 & 39.7 & 15933 & 271814 & 3467 \\
& Tracktor-\motsynth + FT & 56.5 & 78.8 & 52.8 & 11377 & 211772 & 1995 \\
& Tracktorv2~\cite{Bergmann19ICCV} & 52.6 & 79.9 & 52.7 & \textbf{6930} & 236680 & 1648 \\
\cline{2-8}
& CenterTrack-\motsynth & 39.7 & 72.9 & 37.2 & 47066 & 259274 & 5872 \\
& CenterTrack-\motsynth + FT & 41.9 & \textbf{80.2} & 38.2 & 36594 & 258874 & 5313 \\
\cline{2-8}
& MPNTrack~\cite{braso2020learning} & \textbf{57.6 }& 79.0 & 59.1 & 16953 & \textbf{201384} & \textbf{1210}  \\
& LPC~\cite{dai2021learning} & 56.3 & 79.7 & \textbf{62.5} & 11726 & 213056 & 1562  \\
& SORT20~\cite{bewley2016simple} & 42.7 & 78.5 & 45.1 & 27521 & 264694 & 4470  \\
\bottomrule
\end{tabular}}
\vspace{-7pt}
\caption{Benchmark results on MOT17 and MOT20. We refer to supplementary for the full version.}
\label{tab:mot-bench}
\end{table}



==> tables/tracking/mot.tex <==
\begin{table}
\center
\tabcolsep=0.11cm
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|l| c| c |c c c c c c c}
\toprule
& Dataset & FT & ReID & MOTA $\uparrow$ & MOTP $\uparrow$ & IDF1 $\uparrow$ &  TP $\uparrow$ & FP $\downarrow$ & FN $\downarrow$ & IDS $\downarrow$  \\ [0.5ex] 
\midrule
\parbox[t]{3mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{Tracktor~\cite{Bergmann19ICCV}}}} 
& COCO & \xmark & \xmark & 43.5 & 0.192 & 49.6 & 26783 & \textbf{2816} & 27259 & 467 \\ %
& COCO & \xmark & Market1501 & 44.0 & 0.192 & 55.1 & 26783 & \textbf{2816} & 27259 & 179 \\ %
& COCO & \checkmark & Market1501 & 48.3 & 0.193 & 58.1 & 29218 & 27259 & 24824 & 185 \\ %
\cline{2-11}
& \motsynth & \xmark & \xmark & 45.0 & 0.197 & 51.2 & 28749 & 3992 & 25293 & 458 \\ %
& \motsynth & \xmark & Market1501 & 45.5 & 0.197 & 56.8 & 28749 & 3992 & 25293 & 161 \\%slurm-347221.out
& \motsynth & \xmark & \motsynth & 45.5 & 0.197 & 56.8 & 28749 & 3992 & 25293 & \textbf{160}\\%slurm-347221.out
\cline{2-11}
& \motsynth & \checkmark & \xmark & 49.8 & \textbf{0.199} & 53.8 & \textbf{30588} & 3264 & \textbf{23454} & 411 \\ %
& \motsynth & \checkmark & Market1501 & \textbf{50.3} & \textbf{0.199} & 59.8 & \textbf{30588} & 3264 & \textbf{23454} & 167 \\ %
& \motsynth & \checkmark & \motsynth &\textbf{ 50.3} & \textbf{0.199} & \textbf{59.9} & \textbf{30588} & 3264 & \textbf{23454} & 165 \\ %
\midrule
\midrule
\parbox[t]{3mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{CenterTr.~\cite{zhou20ECCV}}}} 
& ImageNet & \checkmark & -- & 60.7 & 0.190 & 62.7 & 35443 & 2179 & 18447 & 564 \\
\cline{2-11}
& CrowdHuman & \xmark & -- & 52.2 & \textbf{0.218} & 53.8 & \textbf{32486} & 3604 & 21404 & 728 \\
& CrowdHuman & \checkmark & -- & 66.1 & 0.179 & 64.2 & 38604 & 2442 & 15286 & 528 \\
\cline{2-11}
& \motsynth & \xmark & -- & 54.3 & 0.205 & 57.7 & 33504 & 3601 & 20386 & 666 \\
& \motsynth & \checkmark & -- & \textbf{67.9} & 0.179 & \textbf{66.5} & 38681 & \textbf{1606} & \textbf{15209} & \textbf{508} \\
\bottomrule
\end{tabular}}
\vspace{-7pt}
\caption{Multi-object tracking results performed on MOT17 training set.}
\label{tab:mot}
\end{table}






==> tables/tracking/mots.tex <==
\begin{table}
\center
\tabcolsep=0.11cm
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|l| c c c c c c c c}
\toprule

& Dataset & sMOTSA $\uparrow$ & MOTSA $\uparrow$ & MOTSP $\uparrow$ & IDF1 $\uparrow$ & TP $\uparrow$ & FP $\downarrow$ & FN $\downarrow$ & IDS $\downarrow$  \\ [0.5ex] 

\midrule


\parbox[t]{3mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\cite{Voigtlaender19CVPR}}}} 
& \multirow{2}{*}{Several} & \multirow{2}{*}{52.74} & \multirow{2}{*}{66.90} & \multirow{2}{*}{80.16} & \multirow{2}{*}{51.19} & \multirow{2}{*}{19202} & \multirow{2}{*}{894} & \multirow{2}{*}{7692} & \multirow{2}{*}{315} \\
&  &  &  &  &  &  &  &  &  \\

\midrule
\parbox[t]{3mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\cite{Bergmann19ICCV}}}}
& COCO & 55.58 & 68.80 & \textbf{81.93} & 63.24 & 19677 & 1016 & 7217 & 159 \\
& \motsynth & 55.54 & 68.73 & \textbf{81.93} & 63.09 & 19626 & 987 & 7268 & 155 \\
& \motsynth$^{\dagger}$ & \textbf{56.10} & \textbf{69.52} & 81.67 & \textbf{67.53} & \textbf{19690} & \textbf{850} & \textbf{7204} & \textbf{143} \\
\midrule
\parbox[t]{3mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\cite{hornakova20ICML}}}}
& COCO & 53.59 & 67.53 & \textbf{81.52} & 73.31 & 20279 & 2026 & 6615 & 92 \\
& \motsynth & \textbf{54.09} & \textbf{68.07} & 81.49 & \textbf{73.48} & \textbf{20304} & \textbf{1912} & \textbf{6590} & \textbf{86} \\

\midrule
\parbox[t]{3mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\cite{zhou20ECCV}}}} 
& COCO & \textbf{53.93} & \textbf{67.49} & 81.68 & \textbf{58.4} & \textbf{19919} & \textbf{1488} & \textbf{6975} & 279 \\
& \motsynth & 53.88 & 67.37 & \textbf{81.74} & 58.19 & 19876 & 1497 & 7018 & \textbf{260} \\




\midrule
\parbox[t]{3mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\cite{braso2020learning}}}} 
& COCO & 48.50 & 62.41 & 81.34 & 69.03 & 20061 & 3177 & 6833 & 99 \\
& \motsynth & \textbf{49.17} & \textbf{63.03} & \textbf{81.44} & \textbf{69.40} & \textbf{20079} & \textbf{3047} & \textbf{6815} & \textbf{82} \\


\bottomrule
\end{tabular}}
\vspace{-7pt}
\caption{Multi-object tracking and segmentation. Masks were generated using Mask R-CNN model, trained on COCO and \motsynth. Baselines: Track R-CNN~\cite{Voigtlaender19CVPR}, Tracktor~\cite{Bergmann19ICCV}, Lift\_T~\cite{hornakova20ICML}, CenterNet~\cite{zhou20ECCV}, MPNTrack~\cite{braso2020learning}}
\label{tab:mots}
\end{table}







==> tables/tracking/mots_bench.tex <==

\begin{table}
\center
\tabcolsep=0.11cm
\resizebox{\columnwidth}{!}{
\begin{tabular}{l| c c c c c c c c}
\toprule

Method & sMOTSA $\uparrow$ & MOTSA $\uparrow$ & MOTSP $\uparrow$ & IDF1 $\uparrow$ & TP $\uparrow$ & FP $\downarrow$ & FN $\downarrow$ & IDS $\downarrow$  \\ [0.5ex] 

\midrule

Tracktor$^{\dagger}$-\motsynth & \textbf{55.1} & \textbf{70.2} & \textbf{79.6} & \textbf{63.9} & \textbf{23994} & \textbf{1128} & \textbf{8275} & \textbf{200} \\
TrackRCNN~\cite{Voigtlaender19CVPR} & 40.6 & 55.2 & 76.1 & 42.4 & 19628 & 1261 & 12641 & 567 \\
\bottomrule
\end{tabular}}
\vspace{-7pt}
\caption{Benchmark results on MOTS20 dataset.}
\label{tab:mots-bench}
\end{table}


